Confidence-Calibrated Ensemble Dense Phrase Retrieval

In this paper, we consider the extent to which the transformer-based Dense Passage Retrieval (DPR) algorithm, developed by (Karpukhin et. al. 2020), can be optimized without further pre-training. Our method involves two particular insights: we apply the DPR context encoder at various phrase lengths (e.g. one-sentence versus five-sentence segments), and we take a confidence-calibrated ensemble prediction over all of these different segmentations. This somewhat exhaustive approach achieves start-of-the-art results on benchmark datasets such as Google NQ and SQuAD. We also apply our method to domain-specific datasets, and the results suggest how different granularities are optimal for different domains

==> FIGURES.tex <==
\begin{table*}[h!]
\begin{center}
\begin{tabular}{m{6cm}m{2cm}m{2cm}m{2cm}m{2cm}|m{2cm}}%{@{}ccccc@{}}
\toprule
 & SQUAD & PubmedQA & SCOTUS & NFCorpus&\\ \hline
 1 & 53.4 & 77.8 & 66.2 & 30.8&   \\
 3 & 44.7 & 76.5 & 65.1 & 24.5&  \\
 5 & 47.0 & 72.7 & 61.4 & 21.9& \\
MUF & 54.5 & 84.8 & 70.0 & 27.8& \\\hline
%\bottomrule
\end{tabular}
\caption{ F-1 scores of dense phrase retrieval evaluated on major datasets based on top 30 evaluation. }
\end{center}
\end{table*}


\begin{table*}[h!]
    \centering
    \begin{tabular}{c|c c}
     & NQ (train) & NQ (dev)\\ \hline
      75   & 70.2 &  77.4 \\%41.3\\
      125   & 69.0 & 74.0 \\
      250 & 65.3 & 70.1 \\
      MUF & 83.0 & 86.7 
    \end{tabular}
    \caption{F-1 scores of dense phrase retrieval evaluated on major datasets based on top 30 evaluation.}
    \label{tab:my_label}
\end{table*}

